Constraining Post-Newtonian Parameters with the Cosmic Microwave Background

The Parameterised Post-Newtonian (PPN) approach is the default framework for performing precision tests of gravity in nearby astrophysical systems. In recent works we have extended this approach for cosmological applications, and in this paper we use observations of the anisotropies in the Cosmic Microwave Background to constrain the time variation of the PPN parameters $\alpha$ and $\gamma$ between last scattering and the present day. We find their time-averages over cosmological history should be within $\sim 20\%$ of their values in GR, with $\bar{\alpha}=0.89^{+0.08}_{-0.09}$ and $\bar{\gamma}=0.90^{+0.07}_{-0.08}$ at the $68\%$ confidence level. We also constrain the time derivatives of these parameters, and find that their present-day values should be within a factor of two of the best Solar System constraints. Many of these results have no counter-part from Solar System observations, and are entirely new constraints on the gravitational interaction. In all cases, we find that the data strongly prefer $\bar{\alpha}\simeq \bar{\gamma}$, meaning that observers would typically find local gravitational physics to be compatible with GR, despite considerable variation of $\alpha$ and $\gamma$ being allowed over cosmic history. This study lays the groundwork for future precision tests of gravity that combine observations made over all cosmological and astrophysical scales of length and time.

==> prev_code_implementation.tex <==
We implement the framework described above by modifying the Cosmic Linear Anisotropy Solving System (CLASS) \cite{lesgourgues2011cosmic}, which is a Boltzmann code that evolves perturbations from early times up to the present day. In particular, we implement the modified Friedmann equation, the momentum constraint equation (used to evolve $\Psi$) and the slip equation (used to calculate $\Phi$). See appendix \ref{app_code} for full details of the implemented equations.

In implementing our approach we necessarily need to make some choices, which we detail here. They are (i) a choice for how to include radiation, and (ii) a choice of how to specify the functional form of the time dependence of the coupling parameters, and (iii) a choice of how to deal with the large-scale slip. None of these are uniquely specified within the PPNC approach. \DBT{This third one isn't really an implementation choice  I think - it is just a parameter we set to its GR value when doing the MCMC.}

The PPNC construction outlined above is constructed by considering the gravitational fields of pressureless dust and dark energy, and does not explicitly include radiation or neutrinos in its present form. This is due to the PPN formalism having been constructed to deal with the gravitational fields of astrophysical bodies in the late Universe, which have mass as the leading-order contribution to the source of their gravitational fields. This is not true for relativistic species such as radiation and neutrinos, for which isotropic pressure also contributes at leading order. In principle, this situation could be remedied by extending the PPN formalism to include such contributions, but we expect this to be a non-trivial task that may involve generalizing the post-Newtonian expansion itself, as well as potentially involving the introduction of additional coupling parameters (see Ref \cite{Sanghai_2016} for preliminary steps). 

For our implementation in the present study we have made what we consider to be the most conservative choice possible; not modifying the gravitational coupling to other species at all, such that (for example) the Friedmann equation in the code appears as
\begin{equation}\label{eqn_Friedmann_code}
    H=\sqrt{\frac{8\pi G}{3}\left(\bar{\rho}_\text{tot}-\bar{\rho}_c-\bar{\rho}_b\right)+\frac {8\pi G}{3}\left(\bar{\rho}_c+\bar{\rho}_b\right)\gamma-\frac{2\gamma_c}{3}}
\end{equation}
where we have taken the curvature of spatial 3-volumes to vanish, and where $\bar{\rho}_\text{tot}$ is the total energy density, and $\bar{\rho}_c$ and $\bar{\rho}_b$ are respectively the energy densities of cold dark matter and baryonic matter, with the source terms of other equations being prescribed similarly. This choice is not unique, but provides us with a definite means to calculate the effect of the change in gravitational coupling strengths of pressureless matter without having to make significant changes to the radiation-dominated stage of cosmic history.

Next on the list above is the functional form of the PPNC parameters $\{\alpha, \gamma, \alpha_c, \gamma_c\} = \{\alpha(\tau), \gamma(\tau), \alpha_c(\tau), \gamma_c(\tau)\}$, which we input directly into the code's initialization file. We choose to specify the time-dependence of $\alpha$ and $\gamma$ by making them functions of the scale factor $a$, in the following way:
\begin{eqnarray} \label{eq_ppnc_power_law_n}
\alpha(a)=A\left(\frac{a_1}{a}\right)^n+B \qquad {\rm and} \qquad    \gamma(a)=C\left(\frac{a_1}{a}\right)^n+D\text{,}
\end{eqnarray}
with the constants $\{A, B, C, D\}$ calculated from the values of $\alpha$ and $\gamma$ at the initialization time $a=a_1$ and at the present time $a=1$ (which is conventionally unity for $\alpha$, and strongly constrained from astrophysical bounds for $\gamma$ \cite{Will_2014,Bertotti_2003}). The value of $n$ can then be used to control the rate of change of the parameters over cosmic history, and in what follows we will consider different values for this quantity. The reader will note that we have chosen the power-law index for both $\alpha$ and $\gamma$ to be the same, which is done for simplicity, and could be easily relaxed. \DBT{Later justification for this choice could be included here.}

\DBT{This following paragraph mixes implementation and specific study choices: gammac constant and large scale slip set to 1 (me note - small scale slip is not set to 1, and interpolation is used).}\\
The dark energy component of the Universe (including $\Lambda$) is included in $\alpha_c$ and $\gamma_c$, and we choose to specify $\gamma_c$ as a constant determined by its fractional contribution to $H$ at $z=0$, so that it appears in the Friedmann equation in a way that is as similar as possible to $\Lambda$. The integrability condition (\ref{eq_integrability}) is then used to specify $\alpha_c$, and we choose to set the value of the large-scale slip to its general-relativistic value of one. This last choice is for convenience in the present study, and can be re-visited if/when a theoretical prediction of this quantity is found for the PPNC framework. It can also be straightforwardly relaxed by including additional parameters, if this should be desired in future studies. For all of the PPNC modifications, we choose to take them as not being present when the initial conditions are set, but rather to switch them on at an arbitrary point deep in the radiation era (at $a_1=10^{-10}$, where their contributions are negligible).\\
\DBT{Moved to here: In addition it makes the $\gamma_c$ contribution to the background largely equivalent to $\Omega_\Lambda$, which is well understood, and our choice also allows us to focus primarily on $\alpha$ and $\gamma$ for this first investigation into the constraints that can be obtained on the PPN parameters from the CMB.}

The power-law form for $\alpha$ and $\gamma$ are chosen for their simplicity, and the smoothness of the functions that result. Treating them as piece-wise functions in bins would not result in the required smoothness, and tying them to dark energy (as in e.g. \cite{planck}) would not appear to be a sensible choice in the present context, as we are interested in precision tests of gravity rather than testing candidates for dark energy. Our power-law approach is supported by the behaviour found in Ref. \cite{Thomas_2023} for some example theories of gravity, where in those cases the same power-law index for $\alpha$ and $\gamma$ was found to be a good description\footnote{A value of $n$ close to 0.1 was a good fit for the theories in Ref. \cite{Thomas_2023} that were furthest from $\Lambda$CDM, which is partly why we choose $n=0.1$ in some of our investigations below.}. 

We anticipate that Gaussian processes or genetic algorithms might be better and more model-independent ways to reconstruct the PPNC functions from observations, but we leave the use of these more sophisticated approaches for future work.

For the purposes of the parameter constraints detailed later, the primary parameters to be constrained are $\gamma(a_1)$, $\alpha(a_1)$ and $n$. In order to reduce the degeneracy between the first two of these with the third, and work with a more physically relevant variable, we  will present our results using the averages of $\alpha$ and $\gamma$ over cosmic time, defined as
\begin{equation} \label{agbar}
\bar{\alpha}\equiv \frac{\int^{0}_{\ln a_1}{\alpha(a)\,\mathrm{d} \ln a}}{\int^{0}_{\ln a_1}{\mathrm{d} \ln a}}
\qquad {\rm and} \qquad
\bar{\gamma}\equiv \frac{\int^{0}_{\ln a_1}{\gamma(a)\,\mathrm{d} \ln a}}{\int^{0}_{\ln a_1}{\mathrm{d} \ln a}}\text{.}
\end{equation}

Two additional derived parameters calculated by the modified Boltzmann code are presented in the MCMC results, which are the derivatives of $\gamma$ and $\alpha$ with respect to the scale factor at the present time ($a=1$). 

The full set of perturbation, background, PPNC functions, and constraint equations, as implemented in the code, and in the notation and conventions used within CLASS, is given in Appendix \ref{app_code}.

\subsection{Relationship to varying $G$}
Varying $G$ tests typically modify a specific equation, derived in a particular context. Modified gravity theories can effectively modify $G$ differently in different contexts, so constraints on $G$ in one context don't apply in other contexts when varying $G$ is being used as a proxy for modified gravity.

As such, varying $G$, and equivalently cosmological tests using $\mu$ as a modification of the Poisson equation in cosmological perturbation theory, are not generally equivalent to constraints on the PPN parameters.\footnote{See e.g. \cite{ppnvscosmo} for related comments on this issue.} One key exception is Solar System tests of $\dot{G}$ that occur in the same weak-field perturbations about Minkowski regime that PPN is designed for. The constraints from these tests on $\frac{\dot{G}}{G}$ are equivalent to a constraint on $\dot{\alpha}$ (at $z\approx0$). A good summary of these tests and associated references is \cite{Will_2014}, with the Mars ephemeris constraints being the strongest,\footnote{Taking this as a constraint on $\dot{\alpha}$ requires assuming that the mass loss from the sun is negligible.} constraining $\dot{\alpha}=\frac{\dot{G}}{G}=0.1\pm1.6 \times 10^{-13} yr^{-1}$, followed by Lunar laser ranging (about five times larger) and Heliosismology (around an order of magnitude larger). Conversely, the big bang nucleosynthesis constraints cited in the same reference\footnote{See e.g. \cite{bbn} for a more recent treatment.} does not correspond to the time variation of the PPN parameters $\alpha$ or $\gamma$, because these constraints come from modifying the background Friedmann equation during the radiation dominated era.

==> theo_section.tex <==
% \subsection{Degeneracies and what is driving the constraints - Theo}

% In this section, we will explore the physical interpretation of the results obtained from the MCMC analyses. We will focus first on the PPNC parameters $\bar{\alpha}$ and $\bar{\gamma}$, and then on their degeneracies with the cosmological parameters, most notably $H_0$ and $\omega_c\,$. Finally, we will briefly discuss the apparent weak preference in the data for the PPNC parameters both being slightly below their GR values of unity.

% \subsubsection{Degeneracy between PPNC parameters}

% One of the most notable features of the posteriors obtained in our MCMC analyses is that in each case $\bar{\alpha}$ and $\bar{\gamma}$ are strongly degenerate, as shown in the triangle plots in Appendix \ref{sec:triangle}.
% Moreover, the 1D posteriors demonstrate that the CMB data we have used indicate a strong preference for $\bar{\alpha}$ and $\bar{\gamma}$ to be roughly equal. In general, the difference $\vert \bar{\alpha} -\bar{\gamma} \vert$ in the posteriors is constrained much closer to zero than either $\vert \bar{\alpha} - 1 \vert$ or $\vert \bar{\gamma} - 1 \vert$ is. 
% \footnote{Note that $\bar{\alpha}$ and $\bar{\gamma}$ being equal means that $\alpha(a) = \gamma(a)\, \forall \, a$, as they have the same power law index $n$, and we are implementing the condition $\gamma(a = 1) = 1$, while $\alpha(a = 1) = 1$ by definition.}

% The fact that $\bar{\alpha} \neq \bar{\gamma}$ is disfavoured is shown by Fig. \ref{fig_mean_residual_0pt1_with_G}, which shows the mean absolute residual, averaged over $l \in \left[2, 1001\right)$, in $\mathcal{C}_l^{TT}$ relative to the best-fit $\Lambda$CDM, for a PPNC power law with $n = 0.1$\,.
% For example, that mean absolute residual is  $80.2\,\%$ for $\left(\bar{\alpha}, \bar{\gamma}\right) = \left(1.15, 0.85\right)$, whereas it is $1.67\,\%$ for $\left(\bar{\alpha}, \bar{\gamma}\right) = \left(0.85, 0.85\right)$, and $1.61\,\%$ for $\left(1.15, 1.15\right)$\,, even though in all of these cases $\vert \bar{\alpha} -1 \vert$ and $\vert \bar{\gamma} - 1 \vert$ are the same. 

% \begin{figure}[h]
% \centering
% \begin{subfigure}{0.45\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/with_G_highres_mean_residual_G_corrected.pdf}
%     \caption{}
%     \label{fig_mean_residual_0pt1_with_G}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/no_G_highres_mean_residual.pdf}
%     \caption{}
%     \label{fig_mean_residual_0pt1_no_G}
% \end{subfigure}
% \caption{Colour map of the mean absolute residual of $\mathcal{C}_l$ relative to $\Lambda$CDM, averaged over multipoles $l \in \left[2,1001\right]$. Results are displayed as a function of $\bar{\alpha}$ and $\bar{\gamma}$, for the $n = 0.1$ PPNC power law. In the left panel, we have used the full set of PPNC equations. In the right panel, the term $\mathcal{G}\mathcal{H}\Psi$ has been artificially removed from the momentum constraint equation, in order to demonstrate the importance of the PPNC $\mathcal{G}$ function in driving $\bar{\alpha} \approx \bar{\gamma}$\,.}
% \label{fig_mean_residual_0pt1}
% \end{figure}

% The degeneracy between $\bar{\alpha}$ and $\bar{\gamma}$, and equivalently the strong preference for $\bar{\alpha} \approx \bar{\gamma}$, can be explained with reference to the PPNC Friedmann equation Eq. \ref{eqn_Friedmann_code}, and the perturbation equations, Eqs. (\ref{eq_pert1}-\ref{eq_pert3}). 
% Eq. \ref{eqn_Friedmann_code} is used in the PPNC-CLASS code to evolve the background evolution. It contains only $\gamma$, and not $\alpha$, which is irrelevant to the background expansion for our choice of $\gamma_c$ time-evolution \footnote{in principle, $\alpha$ could enter into the background if one chose to specify the time evolution of $\alpha_c$ rather than $\gamma_c$, and then calculate the evolution of $\gamma_c$ from the integrability condition Eq. (\ref{eq_integrability}), which contains $\alpha$.}.
% However, the perturbation equations involve both $\alpha$ and $\gamma$, through the interpolating functions $\mu(k, a)$, $\xi(k, a)$ and $\mathcal{G}(k,a)\,$. These are explicitly dependent on the PPNC parameters and their time derivatives, via their functional forms given by Eqs. (\ref{eqn_timinterp0}-\ref{eq_ppnc_curlyG}).

% As the CMB observables depend on the evolution of both the background cosmology, which is sensitive only to $\gamma(a)$, and the metric perturbations, which are sensitive to both $\gamma(a)$ and $\alpha(a)$, it follows that if $\bar{\alpha}$ and $\bar{\gamma}$ are equal, then there must be a ``cancellation'' between the effects of the PPNC system's departures from $\Lambda$CDM on the background, and their effects on the perturbations. We will show shortly that this is indeed the case.
% This cancellation is increasingly broken as $\bar{\alpha} - \bar{\gamma}$ is taken further away from zero. 

% The combination $\alpha - \gamma$ appears explicitly at only one place in the perturbation equations, Eqs. (\ref{eq_pert1}-\ref{eq_ppnc_curlyG}). 
% This is in the term $\mathcal{G}\mathcal{H}\Psi$ in the momentum constraint (\ref{eq_pert3}), which determines the evolution of $\Psi$. 
% In the limit $k \longrightarrow \infty$, corresponding to modes deep inside the horizon, $\mathcal{G}$ is given by $\left(\alpha - \gamma\right)/\gamma + \hat{\gamma}/\gamma\,$, as per Eq. (\ref{eq_ppnc_mu}). 
% The function $\mathcal{G}$ vanishes at all times and for all perturbation wavenumbers in $\Lambda$CDM. If $\alpha = \gamma$, then $\mathcal{G}$ remains small outside of GR, with contributions to it coming only from $\hat{\gamma}/\gamma\,$. Therefore, the explicitly non-GR contributions to Eq. (\ref{eq_pert3}) are suppressed, even if $\gamma = \alpha$ is deviant from unity, and so a $\Lambda$CDM-like CMB power spectrum can be obtained with a suitable set of cosmological parameters.

% By contrast, if $\bar{\alpha} \neq \bar{\gamma}$, then the non-GR term $\mathcal{G}\mathcal{H}\Psi$ drives distinct phenomenology in the CMB, which could push it well outside the Planck error bars no matter how much the basic $\Lambda$CDM parameters are adjusted.

% These considerations lead us to the following three related conjectures:
%     \begin{enumerate}
%         \item If $\bar{\alpha}$ and $\bar{\gamma}$ are equal, then there must be a cancellation between the effects of the background (which only involves $\alpha$) and the perturbations (which involve both $\gamma$ and $\alpha$), so that the overall CMB produced is consistent with the observed spectra.
%         \item the $\mathcal{G}$ function drives the preference for $\bar{\alpha} = \bar{\gamma}$ as it becomes large if they are not equal.
%         \item If $\bar{\alpha}$ and $\bar{\gamma}$ are not equal, then the background-perturbations cancellation does not happen, because the $\mathcal{G}$ function changes the evolution of the perturbations substantially. Hence, the perturbations can no longer cancel off the background.
%     \end{enumerate}

% We will now show that these conjectures correctly explain the observed degeneracy between the PPNC parameters $\bar{\alpha}$ and $\bar{\gamma}\,$.
% First, we consider what happens if one artificially removes the $\mathcal{G}\mathcal{H}\Psi$ term from Eq. (\ref{eq_pert3}), and then re-runs the PPNC-CLASS code without that term, in order to calculate the mean absolute residual in $\mathcal{C}_l$ relative to $\Lambda$CDM, as we previously calculated in Fig. \ref{fig_mean_residual_0pt1_with_G} for the true PPNC equations with this term retained. 
% Fig. \ref{fig_mean_residual_0pt1_no_G} shows that the preference for $\bar{\alpha} = \bar{\gamma}$ is then substantially reduced, with a maximum value of $\left\langle \vert\left(\mathcal{C}_l - \mathcal{C}_l^{\Lambda{\rm CDM}}\right)/\mathcal{C}_l^{\Lambda{\rm CDM}}\vert\right\rangle$ of $24.0\%$ in the corner $\left(\bar{\alpha}, \bar{\gamma}\right) = \left(1.15, 0.85\right)\,$. 

% Next, we consider the effects on $\mathcal{C}_l^{TT}$ of the PPNC background and perturbation evolution, in order to show that there is indeed a cancellation that occurs for $\bar{\alpha} = \bar{\gamma}$, and that this cancellation is worse for $\bar{\alpha} \neq \bar{\gamma}$ (driving the results much further from the Planck best-fit $\Lambda$CDM and making them disfavoured by the data). 
% We will also show that the non-cancellation in the unequal case is driven primarily by the presence of the $\mathcal{G}$ PPNC function.
% To do this, we run the code for a given choice of $n$, $\bar{\alpha}$ and $\bar{\gamma}$ three times: once where the entire system of PPNC equations is used, once where the perturbations are evolved according to the PPNC perturbation equations but the background is evolved with the $\Lambda$CDM Friedmann equations, and once where the perturbations follow $\Lambda$CDM equations but the background follows the PPNC Friedmann equations. 
% We then do this again, but with the term proportional to $\mathcal{G}$ artificially removed from the momentum constraint equation.

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.32\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/TT_background_vs_perturbations_0pt87_0pt87_G.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/Sachs_Wolfe_background_vs_perturbations_0pt87_0pt87_G.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/Doppler_background_vs_perturbations_0pt87_0pt87_G.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}   \includegraphics[width=\linewidth]{theo_plots/TT_background_vs_perturbations_0pt87_1pt13_G.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/Sachs_Wolfe_background_vs_perturbations_0pt87_1pt13_G.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/Doppler_background_vs_perturbations_0pt87_1pt13_G.pdf}
%     \end{subfigure}
%     \caption{The relative effects of a PPNC background evolution and PPNC perturbation evolution on the CMB power spectrum. The total $\mathcal{C}_l^{\rm TT}$, the Sachs-Wolfe and Doppler contributions are all displayed. In each case, we have computed the spectra first using the full set of PPNC equations, and then with the $\mathcal{G}$ PPNC function artificially removed, in order to demonstrate its importance. Results are shown for a power law with $n = 0.1$. Top row: $n = 0.1$ power law, with $\bar{\alpha} = \bar{\gamma} = 0.87\,$. Bottom row: $\bar{\alpha} = 1.13$ and $\bar{\gamma} = 0.87\,$. Red curves show the $\Lambda$CDM results, black the results for a full PPNC evolution, green when the PPNC perturbation equations are used but the background expansion is $\Lambda$CDM, and blue when the background is evolved using the PPNC Friedmann equation but the perturbations are evolved according to $\Lambda$CDM equations.}
% \label{fig_background_vs_perturbations}
% \end{figure}

% The results are shown in Fig. \ref{fig_background_vs_perturbations}, where we have displayed the full $\mathcal{C}_l^{TT}$, as well as the Sachs-Wolfe and Doppler source terms, which are the dominant ones driving the constraint between $\bar{\alpha}$ and $\bar{\gamma}$. This is because the power laws for the PPNC parameters can substantially shift their values from unity at $a_{LS}$, as displayed in Fig. \ref{fig_gamma_of_a_power_laws}. Therefore, they directly affect the metric and velocity perturbations at last scattering.

% Both the PPNC background-only and PPNC perturbations-only cases can individually display very large residuals of $\mathcal{C}_l$ from $\Lambda$CDM. 
% In the case $\bar{\alpha} = \bar{\gamma} = 0.87$ (for an $n = 0.1$ power law), these effects cancel very well, and the power spectrum for the full PPNC system (background and perturbations) remains close to $\Lambda$CDM for all multipoles. 
% This is also true for both the Sachs-Wolfe and Doppler contributions, suggesting an underlying symmetry at the level of the metric perturbations that source those terms. 

% In the case $\left(\bar{\alpha}, \bar{\gamma}\right) = \left(1.13, 0.87\right)$, there is virtually no cancellation. Instead, the effects of the background and perturbations ``add together'' to further amplify the acoustic peaks, and the $l \gtrsim 500$ region is dominated by the PPNC perturbations, which are highly deviant from $\Lambda$CDM.
% However, we see that the non-cancellation in the case $\bar{\alpha} \neq \bar{\gamma}$ is much less severe if we artificially remove the $\mathcal{G}$ term from the PPNC momentum constraint equation, as shown in the right half of each quadrant on the bottom set. For $\bar{\alpha} = \bar{\gamma}$, removing $\mathcal{G}$ has very little effect, as expected.

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.32\textwidth}
%         \includegraphics[width=\linewidth]{theo_plots/effect_of_G_corrected_ppnc_0pt1.pdf}
%         \caption{}
%     \end{subfigure}
%         \begin{subfigure}{0.32\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/effect_of_G_corrected_ppnc_m0pt4.pdf}
%         \caption{}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/effect_of_G_corrected_ppnc_0pt4.pdf}
%         \caption{}
%     \end{subfigure}
    
%     \caption{The effect of the $\mathcal{G}$ PPNC function on the CMB TT power spectrum, for the $n = 0.1$ (left), $n = -0.4$ (middle) and $n = 0.4$ (right) power laws. The top left panel of each quartet shows the spectra themselves, where solid lines correspond to using the full PPNC perturbation equations and dashed lines to removing the $\mathcal{G}\mathcal{H}\Psi$ term from the momentum constraint equation. The top right, bottom left and bottom right panels show the total residual relative to $\Lambda$CDM, the residual in the Sachs-Wolfe term and the residual in the Doppler term respectively.}
%     \label{fig_effect_of_G}
% \end{figure}

% Fig. \ref{fig_effect_of_G} further shows the effect of removing the $\mathcal{G}$ term on the overall $\mathcal{C}_l$, and the Sachs-Wolfe and Doppler terms, for three different power laws: the $n = 0.1$ case as above, and also the cases $n = -0.4$ and $n = 0.4$\,.
% The conclusion that without $\mathcal{G}$, the preference for $\bar{\alpha} \approx \bar{\gamma}$ is far weaker, is shared by both the $0.1$ and $-0.4$ power laws. For these, the PPNC parameters are sufficiently far from 1 at last scattering. 
% However, for the $n = 0.4$ power law, removing $\mathcal{G}$ does not have a noticeable effect, and moreover there is no statistically significant preference for $\left(\bar{\alpha}, \bar{\gamma}\right) = \left(0.87, 0.87\right)$ over $\left(1.13, 0.87\right)\,$. They both give rise to results that are nearly indistinguishable from $\Lambda$CDM. 
% This is because for that power law, virtually all the evolution in $\alpha(a)$ and $\gamma(a)$ happens for $a \ll a_{\rm LS}$, as seen in Table \ref{table_equality_LS}.
% Hence, there is very little constraining power on $\bar{\alpha}$ and $\bar{\gamma}$, and no particular need for them to be close together, because by the time of matter-radiation equality, $\alpha$ and $\gamma$ have already relaxed to within $0.3\%$ of unity.

% \begin{table}
%     \centering
% \begin{tabular}{|c|c|c|c|c|c|c|} 
%  \hline 
% Power law index $n$ & $\bar{\gamma}$ & $\bar{\alpha}$ & $\gamma_{\rm eq}$ & $\alpha_{\rm eq}$ & $\gamma_{\rm LS}$ & $\alpha_{\rm LS}$ \\ \hline 
% $0.1$ & $0.87$ & $1.13$ & $0.9439$ & $1.0562$ & $0.9548$ & $1.0452$ \\
% \hline
% $-0.4$ & $0.87$ & $1.13$ & $0.8598$ & $1.1402$ & $0.8631$ & $1.1369$ \\
% \hline
% $0.4$ & $0.87$ & $1.13$ & $0.9970$ & $1.0030$ & $0.9982$ & $1.0019$ \\
% \hline
%  \end{tabular} \\ 
%     \caption{Values of $\gamma$ and $\alpha$ at matter-radiation equality and last scattering.}
%     \label{table_equality_LS}
% \end{table}


% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.42\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/Phi_Psi_ls_k=1e-2_G.pdf}
%     \caption{}
%     \end{subfigure}
%     \begin{subfigure}{0.42\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/Phi_Psi_ls_k=1e-3_G.pdf}
%     \caption{}
%     \end{subfigure}
%     \begin{subfigure}{0.42\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/Phi_Psi_ls_k=1e-4_G.pdf}
%     \caption{}
%     \end{subfigure}
%     \begin{subfigure}{0.42\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/Phi_Psi_ls_k=1e-5_G.pdf}
%     \caption{}
%     \end{subfigure}
%     \caption{Metric perturbations $\Phi$ and $\Psi$ at last scattering, as a function of $\bar{\gamma}$, for $k = \left\lbrace 10^{-2}, 10^{-3}, 10^{-4}, 10^{-5}\right\rbrace \,{\rm Mpc}^{-1}$. They are evaluated for the case where the full PPNC equations are used, for the case where only the perturbations are governed by PPNC equations (and the background by $\Lambda$CDM equations), and for the case where only the background is governed by PPNC equations (and the perturbations by $\Lambda$CDM equations). In these plots, we have set $\bar{\alpha} = \bar{\gamma}$, and have normalised each perturbation by its $\Lambda$CDM value at $z_{LS}$. Results are shown for the $n = 0.1$, $n = -0.4$ and $n = 0.4$ power laws.}
%     \label{fig_Phi_Psi_LS}
% \end{figure}

% The presence of the function $\mathcal{G}$ gives a good explanation as to why $\alpha \neq \gamma$ provides a poor fit to the CMB. However, we have not yet established the converse: why $\alpha \approx \gamma$ provides a good fit, even if that shared value can be rather deviant from its GR value of 1. 
% To understand why this is the case, we recall that the key modifications to the CMB from the PPNC equations occur in the Sachs-Wolfe and Doppler source terms. These are directly sensitive to the values of the scalar metric perturbations $\Phi$ and $\Psi$ themselves at last scattering.
% These are displayed in Fig. \ref{fig_Phi_Psi_LS}, as a function of $\bar{\gamma} = \bar{\alpha}$, for the $n = 0.1$, $-0.4$ and $0.4$ power laws. 

% The horizon scale at last scattering depends on the PPNC parameters and power-law index chosen, but it is typically around $k_H^{\rm LS} \sim 4 \ {\rm or} \ 5 \times 10^{-3}\,{\rm Mpc}^{-1}$ (e.g. $k_H^{\rm LS} = 4.81 \times 10^{-3}\,{\rm Mpc}^{-1}$ in $\Lambda$CDM, and $k_H^{\rm LS} = 4.51 \times 10^{-3}\,{\rm Mpc}^{-1}$ for a PPNC power law with $n = -0.4$ and $\bar{\gamma} = 0.85\,$).
% We consider perturbation wavenumbers ranging from deep inside the horizon to far above it. 
% If $\alpha = \gamma$, then the PPNC modifications to the background and perturbation equations have roughly equal and opposite effects on the gravitational potentials at last scattering. 
% The reason why the effects are opposite is that if $\gamma > 1$, then the coupling $\mu$ to matter in the perturbation equations (\ref{eq_pert1}) and (\ref{eq_pert3}) is larger, and so the growth of perturbations is enhanced. 

% However, $\gamma > 1$ means that for the same total matter density $\bar{\rho}_m$, the expansion rate $H$ is faster, according to Eq. (\ref{eqn_Friedmann_code}). The growth of perturbations is therefore suppressed \TA{by the same amount. Why?}.
% All departures from $\Lambda$CDM are far smaller for $n = 0.4$, for which even at the extremal cases $\vert \bar{\alpha} - 1 \vert = 0.15$ or $\vert \bar{\gamma} - 1 \vert = 0.15$ , both $\alpha$ and $\gamma$ are within $0.3\%$ of unity by last scattering.

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.32\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/effect_of_gamma_0pt1_G.pdf}
%     \caption{}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/effect_of_gamma_m0pt4_G.pdf}
%     \caption{}
%     \end{subfigure}
%     \begin{subfigure}{0.32\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/effect_of_gamma_0pt4_G.pdf}
%     \caption{}
%     \end{subfigure}
%     \caption{The average residual, relative to $\Lambda$CDM, in the Sachs-Wolfe and Doppler terms, for $l \in \left[2, 1001\right]$, as a function of $\bar{\gamma}$. The Sachs-Wolfe and Doppler terms are evaluated for the case where the full PPNC equations are used, for the case where only the perturbations are governed by PPNC equations (and the background by $\Lambda$CDM equations), and for the case where only the background is governed by PPNC equations (and the perturbations by $\Lambda$CDM equations). In these plots, we have set $\bar{\alpha} = \bar{\gamma}$. Results are displayed for the $n = 0.1$, $n = -0.4$ and $n = 0.4$ power laws.}
%     \label{fig_effect_on_SW_Doppler}
% \end{figure}

% Fig. \ref{fig_effect_on_SW_Doppler} displays the effects of the PPNC modifications to the background and perturbations in the mean absolute deviation of $\mathcal{C}_l$ from $\Lambda$CDM, in both the Sachs-Wolfe and Doppler terms.
% Like in Fig. \ref{fig_Phi_Psi_LS}, they are shown as a function of $\bar{\gamma}$ and where we have set $\bar{\alpha} = \bar{\gamma}$\,. Again, we consider the $0.1$, $-0.4$ and $0.4$ power laws. 
% The cancellation, for $\bar{\alpha} = \bar{\gamma}$, between the departures of the background and perturbations from $\Lambda$CDM clearly follows the pattern of the cancellations in modifications to the metric perturbations $\Phi$ and $\Psi$ at last scattering, which is expected because the Sachs-Wolfe term is almost entirely determined by $\Phi_{\rm LS}$, and the Doppler term is also determined by it through the Euler equation evaluated at $a_{\rm LS}\,$.

% Hence, the value of $\bar{\gamma}$ is fairly weakly constrained, and allowed to be quite substantially deviant from 1. It is the difference between the PPNC parameters that is strongly constrained by the data, not their sum or average. 
% \TA{This explains why $\bar{\alpha}$ and $\bar{\gamma}$ are allowed by the data to deviate by between $2\sigma$ and $3\sigma$ from unity, in the chains where the power law index is fixed to be $\leq 0.25\,$}\footnote{For the chains with $n = 0.4$, $0.55$ and $0.7$, the best-fit values of $\bar{\alpha}$ and $\bar{\gamma}$ correspond to the PPNC parameters being so close to unity by $a_{\rm eq}$ that the discussion above is rendered irrelevant.}.
% We will discuss in due course why those deviations are not only allowed, but actually appear, with a mild overall preference for $\bar{\alpha}$ and $\bar{\gamma}$ both being below unity.

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.4\textwidth}
%     \includegraphics[width = \linewidth]{theo_plots/powerlaw_m0pt4_momentum_ls_G_corrected.pdf} 
%     \caption{}
%     \label{fig_G_ppnc_last_scattering_1}
%     \end{subfigure}
%     \begin{subfigure}{0.4\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/powerlaws_momentum_ls_alpha-gamma_G_corrected.pdf}
%     \caption{}
%     \label{fig_G_ppnc_last_scattering_2}
%     \end{subfigure}
%     \caption{Left: colour map in the $\bar{\alpha}-\bar{\gamma}$ plane, showing the absolute value at last scattering of the purely gravitational term $q_{\rm grav} = \mathcal{G}\mathcal{H}\Psi$ in the momentum constraint equation, compared to the sum of the conventional momentum-like terms arising from matter ($q_{\rm mat} = 4\pi G a^2  \mu \left[\bar{\rho}_c v_c + \bar{\rho}_b v_b\right]$) and radiation ($q_{\rm rad} = 4\pi G a^2 \left[\left(\bar{\rho}_{\gamma}+\bar{p}_{\gamma}\right) v_{\gamma} + \left(\bar{\rho}_{\rm ur}+\bar{p}_{\rm ur}\right) v_{\rm ur}\right]$). The wavelength of the perturbations is set equal to the Hubble horizon at last scattering, and results are shown for an $n = -0.4$ power law. 
%     Right: the ratio $q_{\rm grav}/\left(q_{\rm mat} + q_{\rm rad}\right)$ for $k = k_H$ at last scattering, displayed as a function of the difference between the average PPNC parameters, $\bar{\alpha}-\bar{\gamma}$\,. We have set $\bar{\alpha}+\bar{\gamma}$ equal to 2, so that this is essentially a slice of the left plot (and its equivalents for four other power law indices $n$) through the line $y = -x\,$.}
%     \label{fig_G_ppnc_last_scattering}
% \end{figure}

% In Fig. \ref{fig_G_ppnc_last_scattering}, we demonstrate explicitly that the cancellations seen in Figs. \ref{fig_effect_on_SW_Doppler} and \ref{fig_Phi_Psi_LS} are primarily a result of the term $\mathcal{G}\mathcal{H}\Psi$ in the momentum constraint being small when $\bar{\alpha} = \bar{\gamma}$. 
% This is done by Fig. \ref{fig_G_ppnc_last_scattering_1}. It shows that the $\mathcal{G}\mathcal{H}\Psi$ term makes a $\lesssim 2\%$ relative contribution to the momentum constraint at last scattering for the $n = -0.4$ power law whenever $\bar{\alpha} = \bar{\gamma}$ in the range considered, but can contribute up to $20\%$ at the corners where $\vert \bar{\alpha} - \bar{\gamma}\vert$ is maximised. A cut through this colour map is provided in Fig. \ref{fig_G_ppnc_last_scattering_2}, along with cuts of equivalent maps for other power law indices $n$. 
% The contribution of $\mathcal{G}\mathcal{H}\Psi$ to the evolution of horizon-scale perturbations at last scattering is most sensitive to $\bar{\alpha} - \bar{\gamma}$ for $n < 0$, and very insensitive for $n \gtrsim 0.4\,$. 
% This reiterates the point we have made that the requirement $\alpha \approx \gamma$ is most stringent if the PPNC parameters are allowed to be noticeably deviant from GR until well after last scattering, whereas there is very little constraining power in the data if all the deviations from GR are happening in the very early Universe during radiation domination.

% \begin{figure}[h]
%     \centering
% \includegraphics[width=0.65\linewidth]{theo_plots/G_corrected_last_scattering.pdf}
%     \caption{Upper panel: ratio $q_{\rm grav}/\left(q_{\rm mat} + q_{\rm rad}\right)$, as a function of $k$, evaluated at last scattering. Lower panel: $\Phi + \Psi$ as a function of $k$, also at last scattering. The results are shown for $\Lambda$CDM and for the $n = 0.1$, $n = -0.4$ and $n = 0.4$ PPNC power laws. For the PPNC cases, we have used $\bar{\alpha} =1\,$, and $\bar{\gamma}$ is determined by the central value from the posterior when $n$ in the MCMC was fixed to the specified value. The horizon scale at last scattering for each case is also displayed on both plots.}
%     \label{fig_G_last_scattering_k}
% \end{figure}

% Finally, Fig. \ref{fig_G_last_scattering_k} shows the persistence of the effect of the purely non-GR term $\mathcal{G}\mathcal{H}\Psi$ across a wide range of scales at last scattering, for $\bar{\gamma} \neq \bar{\alpha} = 1$. It affects all $k \gtrsim k_H$, at the level of several percent in both the momentum constraint equation and the metric perturbations $\Phi$ and $\Psi$ themselves, as demonstrated by the upper and lower plots respectively. 

% That effect on the potentials is a roughly uniform amplification of the Weyl potential $\Phi + \Psi$ across sub-horizon $k$ scales, when $\bar{\gamma} < \bar{\alpha} = 1\,$. 
% For $\bar{\gamma} < \bar{\alpha}$, $\mathcal{G}(a_{\rm LS}, k_H^{\rm LS}) > 0$. Consider moving the $\mathcal{G}\mathcal{H}\Psi$ term to the left hand side of the momentum constraint equation (\ref{eq_pert3}), so that the LHS is $\Psi' + \mathcal{H}\left(\Phi - \mathcal{G}\Psi\right)$. The damping term is reduced for positive $\mathcal{G}\,$, and therefore the potential $\Psi$ is amplified. Then so is $\Phi$, due to the slip relation $\Phi \approx \frac{\alpha - \gamma}{\gamma}\,\Psi$ on small scales.
% Hence, it its perhaps most natural to think of the novel term $\mathcal{G}\mathcal{H}\Psi$ as a sub-horizon modification to the left hand side of the momentum constraint, that depending on its sign may either increase or decrease the damping of $\Psi'\,$, rather than as an additional ``gravitational'' contribution to the momentum density that affects the evolution of scalar perturbations. The modified damping becomes significant after matter-radiation equality, as $\alpha(a)$ and $\gamma(a)$ couple only to matter. 

% %\TA{Timescales affected by $\mathcal{G}$. Best shown by \ref{fig_momentum_constraint_Phi+Psi}, which is in the appendix at the moment. Doesn't make a difference to $\Phi + \Psi$ before $a \sim 10^{-4}\,$, i.e during radiation domination. Then its effect on sub-horizon perturbations doesn't change much with time from about last scattering onwards. Obviously for super-horizon perturbations it doesn't make a difference because $\mathcal{G}$ goes to zero on super-horizon scales.}

% \subsubsection{Degeneracy between PPNC and cosmological parameters}

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/power_law_chains_none_G.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/power_law_chains_H0_G.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/power_law_chains_H0_omc_G.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/power_law_chains_H0_omc_As_G.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/power_law_chains_H0_omc_As_ns_G.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.48\textwidth}
%     \includegraphics[width=\linewidth]{theo_plots/power_law_chains_all_G.pdf}
%     \end{subfigure}
%     \caption{CMB $TT$ power spectrum $\mathcal{D}_l = l\left(l+1\right)\mathcal{C}_l/2\pi$, shown for the best-fit $\Lambda$CDM parameters from Planck 2018, and for the $n = 0.1$ and $n = -0.4$ PPNC power laws, with their best-fit values of $\bar{\alpha}$ and $\bar{\gamma}$. 
%     We have also shown the Planck 2018 data points. In the first plot, all the basic $\Lambda$CDM cosmological parameters have been fixed for the PPNC curves. 
%     In the second, $H_0$ has been adjusted for the PPNC curves to its best-fit value for each power law, but all the other basic parameters have been fixed to their $\Lambda$CDM values. 
%     In the third, both $H_0$ and $\omega_c = \Omega_c h^2$ have been adjusted, in the fourth $H_0$, $\omega_c$ and $A_s$\,, and in the fifth $H_0$, $\omega_c$, $A_s$ and $n_s\,$. In the sixth, all the basic parameters have been adjusted (i.e. those above, plus $\omega_b$, $\tau_{\rm reio}$ and $YHe\,$. 
%     The PPNC curves have all been shifted by $\mathcal{D}_l^{\rm PPNC} \longrightarrow \mathcal{D}_l^{\Lambda {\rm CDM}} + 5\left(\mathcal{D}_l^{\rm PPNC} - \mathcal{D}_l^{\Lambda {\rm CDM}}\right)$ in order to make the deviations from $\Lambda$CDM more visible. The Planck error bars have been similarly enlarged by a factor of $5$\,.}
%     \label{fig_Cl_1_adjust_parameters}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{theo_plots/gamma_H0_omc.pdf}
%     \caption{Comparison of the effect on the cosmological background expansion of varying $\bar{\gamma}$ (i.e. changing gravity) while holding all the standard $\Lambda$CDM parameters fixed (black), to the effect of varying $\bar{\gamma}$ by the same amount but adjusting $H_0$ (red), or both $H_0$ and $\omega_c$ (green), to compensate its effect on the FLRW expansion.
%     We have displayed results for the $n = 0.1$ (solid) and $n = -0.4$ (dashed) power laws, with $\bar{\gamma} = 0.85$\,, so that the curves $\gamma(a)$ for each power law are as given in Fig. \ref{fig_gamma_of_a_power_laws}. We show the curves $\left\lbrace \theta(a), H(a), \tau(a)\right\rbrace$\,, for $a \in \left[10^{-5}, 1\right]\,$, where $\theta(a) = r_s(a)/d_A(a)\,$. 
%     All curves have been normalised by their $\Lambda$CDM evolution. The quantities $\theta(a_{\rm LS})$ and $\tau(a_{\rm eq})$ respectively determine the locations and heights of the CMB acoustic peaks.}
%     \label{fig_background_gamma_H0_omc}
% \end{figure}

% The most substantial constraint from the data is the requirement $\bar{\alpha} \approx \bar{\gamma}$, which is common to all the chains. 
% There is still clearly some remaining constraining power - not all sets of parameters $\left\lbrace H_0, \omega_c, \omega_b, \tau, A_s, n_s, {\rm Y He}\right\rbrace$ perform equally well. 
% The constraints on those remaining parameters (the standard $\Lambda$CDM cosmological parameters plus YHe, which must be included, as discussed in Section \ref{sec:mcmc}) are not independent from $\bar{\alpha}$ and $\bar{\gamma}$.
% The most significant degeneracies are between $\bar{\alpha}$ and $H_0$, and between $\bar{\gamma}$ and $H_0$. The next-strongest degeneracies are between $\bar{\alpha}$ and $\omega_c$, and between  $\bar{\gamma}$ and $\omega_c$\,. 
% %Any remaining degeneracies with the other standard cosmological parameters that we vary in the MCMC, $\omega_b$, $\tau$, $A_s$, $n_s$ and {\it Y He}, are much smaller.

% Before we go on, we remind the reader that the cosmological expansion is sensitive to $\gamma(a)$ but not $\alpha(a)$, given our choice of PPNC implementation which was explained in Section \ref{subsec:code_implementation}. 
% Therefore, what we are really dealing with are the degeneracies between $\bar{\gamma}$ and $H_0$, and between $\bar{\gamma}$ and $\omega_c$. 
% The requirement $\bar{\alpha} \approx \bar{\gamma}$, which is required by the evolution of the gravitational perturbations, as discussed in detail above, then means that the degeneracies between $\bar{\gamma}$ and $H_0$, and between $\bar{\gamma}$ and $\omega_c$, give rise to roughly the same degeneracies between $\bar{\alpha}$ and $H_0$, and between $\bar{\alpha}$ and $\omega_c$\,.

% The hierarchy of residuals can be seen through the effect of varying these parameters on the temperature $\mathcal{C}_l\,$s themselves, as displayed in Fig. \ref{fig_Cl_1_adjust_parameters}. 
% We show $\mathcal{C}_l^{\rm TT}$ for the $n = 0.1$, $n = -0.4$ and $n = 0.4$ PPNC power laws, where $\bar{\alpha}$ and $\bar{\gamma}$ are set by their best-fit values for the chains with that fixed power law.
% First, we keep all the standard cosmological parameters at their $\Lambda$CDM best-fit values. Then we successively adjust first just $H_0$, then both $H_0$ and $\omega_c$, then all the rest of the $\Lambda$CDM parameters, to their best-fit values from the MCMC.

% The change between the plot with all the standard parameters fixed and the plot with $H_0$ adjusted shows how the PPNC parameters compete with $H_0$ to set the locations of the acoustic peaks. 
% This is because, once $\bar{\alpha}$ has been fixed to be approximately equal to $\bar{\gamma}$, the most significant remaining difference in the CMB power spectrum between the PPNC case and $\Lambda$CDM is that the evolving $\gamma(a)$ modifies the angular diameter distance to last scattering, and the sound horizon at last scattering. Therefore, $\gamma(a)$ generically causes a shift in the peak locations, through the ratio $\theta(a_{\rm LS}) = r_s(a_{\rm LS})/d_A(a_{\rm LS})\,$, unless the changes to $d_A(a_{\rm LS})$ and $r_s(a_{\rm LS})$ conspire to cancel, which does not typically occur.

% The effect of the PPNC power law evolution of $\gamma(a)$ on the cosmological background is demonstrated by Fig. \ref{fig_background_gamma_H0_omc}.
% The reason for the degeneracy between $\bar{\gamma}$ and $H_0$ is indicated by the first set, where, of the standard cosmological parameters, only $H_0$ can be varied. 
% Consider the fourth subplot in particular, which shows $\theta(a)$ relative to $\Lambda$CDM\,. The black curves show the effect of varying $\bar{\gamma}$ while holding all the standard cosmological parameters fixed, whereas the red curves show the effect of varying $\bar{\gamma}$ while also compensating its effect by varying $H_0\,$ \footnote{The brown vertical line indicates $a_{\rm LS}\,$.}. 
% Without adjusting $H_0$, setting $\bar{\gamma} < 1$ shifts $\theta(a_{\rm LS})$ above its $\Lambda$CDM value, corresponding to a lower $l$ for the first acoustic peak. However, it can be compensated by reducing $H_0$ relative to $\Lambda$CDM, as seen in the third subplot, so that the peak locations return to their observed values. This explains the positive degeneracy between $\bar{\gamma}$ and $H_0$. 
% Note, however, that since our fixed power-law analyses tend to indicate a preference for $\bar{\gamma} < 1\,$, they therefore also push $H_0$ to lower values than the $\Lambda$CDM Planck best-fit, with negative implications for the Hubble tension.

% Now, let us focus on the next-strongest degeneracy in our hierarchy, which is the negative degeneracy between $\bar{\gamma}$ and $\omega_c$ (and thus between $\bar{\alpha}$ and $\omega_c$ due to the approximate equality of $\bar{\alpha}$ and $\bar{\gamma}$). 
% Fig. \ref{fig_Cl_1_adjust_parameters} shows that the main effect of adjusting $\omega_c$ is to compensate the effect of the evolution of $\gamma$ on the heights of the acoustic peaks. This can be explained through the second set of plots in Fig. \ref{fig_background_gamma_H0_omc}.
% We focus in particular on the conformal time $\tau$ that has elapsed at a given $a$ since the beginning of the PPNC evolution at $a_1 = 10^{-10}\,$, which is shown in the second subplot as a ratio of its $\Lambda$CDM value. Of particular importance is $\tau_{\rm eq} = \tau(a_{\rm eq})\,$, the matter-radiation equality scale.
% Setting $\bar{\gamma} < 1$ increases $\tau_{\rm eq}\,$, because weakening gravity at the level of the background means that the effective energy density of cold dark matter, $\gamma \rho_c\,$, that enters into the Friedmann equation (\ref{eqn_Friedmann_code}), is always lower than in $\Lambda$CDM.
% Thus, the radiation era lasts longer in $\tau$, and so acoustic oscillations in the photon-baryon fluid have more time to drive acoustic anisotropies in the CMB, before dark matter takes over and suppresses the oscillations.
% Such an amplification of the acoustic peaks is of course entirely equivalent to the effect of lowering $\omega_c\,$ within $\Lambda$CDM. Hence, the effect on $\tau_{\rm eq}$ of reducing $\bar{\gamma}$ from unity can be compensated, at least in part, by a suitable increase in $\omega_c\,$, as seen from the green curves in the same subplot. This explains the negative degeneracy between $\bar{\gamma}$ and $\omega_c\,$.



% %\subsubsection{Preference for weak gravity}

% %\begin{figure}[h]
%  %   \centering
%   %  \includegraphics[width=0.75\linewidth]{theo_plots/low_ell_adjust_params.pdf}
%    % \caption{The same plots as in Fig. \ref{fig_Cl_1_adjust_parameters}, zoomed in on the low-$l$ multipoles, $l \in \left[2, 40\right)\,$.}
%     %\label{fig_Cl_low_ell_adjust_parameters}
% %\end{figure}

% %An interesting feature of the fixed-$n$ chains is they mostly exhibit a mild preference for gravity being weaker than GR in the past, in that $\bar{\alpha}$ and $\bar{\gamma}$ are typically around $2\sigma$ below unity. This is far from a detection. It goes away completely when the power law index is left as a free parameter, in which case there is very little constraining power on the PPNC parameters. However, it is worth understanding, particularly seeing as it relates to some of the constraints that cannot be pinned down entirely to PPNC parameter degeneracies with $H_0$ and $\omega_c\,$.

% %\begin{figure}
%  %   \centering
%   %  \includegraphics[width=0.8\linewidth]{theo_plots/low_ell_adjust_params.pdf}
%    % \caption{Low-$l$ multipoles of $\mathcal{C}_l^{TT}\,$, shown for the PPNC power laws $n = 0.1$ (blue), $n = -0.4$ (green) and $n = 0.4$ (brown), with the values of $\bar{\gamma}$, $\bar{\alpha}$ and the standard $\Lambda$CDM cosmological parameters given by their best-fit values from the relevant fixed power law MCMC analysis. We have also displayed the results for the best-fit Planck $\Lambda$ cosmology, and the Planck 2018 data points, in red. All deviations from $\Lambda$CDM, including the Planck error bars, have been enlarged by a factor of 5. In the second subplot, $H_0$ has been adjusted to compensate the effects of PPNC on the FLRW background; in the third subplot both $H_0$ and $\omega_c$ are adjusted, and in the fourth subplot all the standard $\Lambda$CDM parameters are adjusted.}
%  %   \label{fig_low_ell_multipoles_powerlaws}
% %\end{figure}

% %\TA{It is illuminating to consider the set of $TT$ power spectra displayed in Fig. \ref{fig_Cl_1_adjust_parameters}, where for the $n = 0.1$, $-0.4$ and $0.4$ power laws we successively adjusted $H_0$, $\omega_c$ and then the rest of the standard cosmological parameters. Specifically, we now zoom in on the low-$l$ multipoles, as shown in Fig. \ref{fig_low_ell_multipoles_powerlaws}. The bottom right panel shows that once the remaining parameters are suitably adjusted, the PPNC $n = 0.1$ and $n = -0.4$ power laws provide an overall suppression of power on large scales, relative to $\Lambda$CDM with its Planck best-fit parameters. This reduction in the large-scale power (i.e. the height of the Sachs-Wolfe plateau) is driven by $\alpha$ and $\gamma$ both being lower than $1$ at last scattering for those sets of PPNC parameters, so that the large-scale metric perturbations are smaller than in $\Lambda$CDM. The total power in the low-$l$ multipoles measured by Planck, and previously WMAP, is known to be lower than is expected in vanilla $\Lambda$CDM \cite{Efstathiou_2010,schwarz2016cmb}. Hence, when we include the time-averaged PPNC parameters as free parameters in an MCMC, the results are driven towards values of $\bar{\alpha}$ and $\bar{\gamma}$ below unity, which more closely produce the observed feature of lower-than-expected power on large scales.}


% \begin{itemize}
%     %\item $\alpha$ - $\gamma$ degeneracy
%     %\item PPNC - LCDM degeneracies ($H_0$, $\omega_m$)
%     \item Change to degeneracies with different powerlaws
%     \item Preference for $\bar{\alpha}$ and $\bar{\gamma}$ below 1?
%     %\item With our choices, only $\gamma$ affects the background (see $\alpha_c, \gamma_c$ implementation choice discussion)
%     %\item In terms of the source functions, PPNC parameters primarily affect the Doppler and Sachs-Wolfe terms
%     %\item $\mathcal{G}$ term in momentum constraint causes significant departure from LCDM behaviour if $\alpha\neq\gamma$. The behaviour of the perturbations drives this behaviour. This is the primary reason these are constrained to be approximately equal. (Figs 4, 6-8, 14-15. Also fig 2 to show that closer to LCDM when PPNC parameters are equal).
%     \item When $\alpha\approx\gamma$, the phenomenology has several aspects that combine to give the degeneracy with LCDM parameters:\\
% (A) The effect of the PPNC modifications to the background and perturbations have roughly equal and opposite effects on the gravitational potentials at last scattering. Opposite because larger $\gamma$ increases the growth in the perturbation equation, but also results in larger expansion for the same density. \DBT{Do we have a good argument for the approximately equal magnitudes? Is this something like a Taylor expansion about LCDM?}\\
% (B) The equal and opposite effects on the potentials cause a substantial cancellation of the differences to LCDM, particularly as the key source terms are the Sachs-Wolfe and Doppler terms. The remaining difference to LCDM is the change to the angular diameter distance to last scattering, hence the degeneracy with $H_0$ (improved peak locations when $H_0$ adjusted).\\
% (C) The remaining difference to LCDM is mostly changes to the peak heights, and thus a degeneracy with $\omega_c$. These two are the primary LCDM degeneracies and allow the majority of PPNC changes to be compensated when $\alpha=\gamma$. \\
% (D) The remaining difference is a reduction in the large scale power/Sachs-Wolfe plateau compared to LCDM - this is a known thing within LCDM, so probably this accounts for the (not significant) non-LCDM preference. \DBT{Can we check/quantify this?}

% \item Extent of the above phenomenology? I.e. how far can PPNC parameters differ from LCDM with the cancellation still happening and just a background degeneracy with LCDM, how equal do the parameters need to be to get the approximate cancellation, and what range of powerlaws does it apply for.
% %\item Extra phenomenology: more detail on $\cal{G}$ - which scales are affected, at which times, what effect it has on the perturbations, 
% \end{itemize}



% %\subsection{Figures}
% %\begin{itemize}
%  %   \item Fig 2 - Do zoom in (in terms of colour bar) on top left plot. Showing that $\alpha=\gamma$ makes things closer to LCDM. \DBT{Might be muddied by lack of compensation from known LCDM degeneracies.}
%   %  \item Fig 3 - NEEDED? Source terms kinda prefer $\alpha=\gamma$. SW changes the most then Doppler. SW/Doppler colour-map patterns very similar.
%    % \item Fig 4 - NEEDED? $\mathcal{G}$ drives non-LCDM behaviour - when it is switched off, don't require $\alpha=\gamma$ to get close to LCDM.
%     %\item Fig 5 - Not needed for paper.
%     %\item Fig 6 - Effect of $\mathcal{G}$ on Cls \& source functions. On/off doesn't matter for $\alpha=\gamma$; lookd like LCDM for $\alpha=\gamma$; wild deviations otherwise; similar story for 2 powerlaws.
%     %\item Figs 7 \& 8 When $\alpha=\gamma$, background are equal and opposite and largely cancel (total is close to LCDM). When they aren't equal the total PPNC change is dominated by the perturbations. There is a residual change to the perturbations when $\alpha\neq\gamma$ and $\mathcal{G}$ is artificially turned off, but this won't drive the behaviour we see (subdominant to the effect from $\mathcal{G}$). (blue is PPNC only for background, red is LCDM, black is total, green is PPNC only for perturbations)
%     %\item Fig 9 - Background quantities for different powerlaws - expand and link to difference in degeneracies for different powerlaws. We should possibly comment on $H_0$ tension based on these plots.
%     %\item Fig 11 - Background and perturbation contributions to SW \& Doppler are equal and opposite as $\bar{\gamma}$ varies for $\alpha=\gamma$. This applies for two different power laws (but cancellation good over smaller range for $n=-0.4$).
%    % \item Fig 12 - It is the effect on the potentials that really cancels (shown for $n=0.1$)
%     %\item Fig 13 - Compensating PPNC effects with $H_0$ \& $\omega_c$ to explain degeneracy, for two different powerlaws. $H_0$ does more of the compensation, and this is even more true for $n=0.1$.
%     %\item Fig 14 - Shows that $\mathcal{G}$ term is large at last scattering if $\alpha\neq\gamma$.
%    % \item Fig 15 - Effect of $\alpha\neq\gamma$ on $\mathcal{G}$ \& potentials at last scattering. Primarily sub-horizon effect. Larger for $n=-0.4$ - see if this is due to $\bar{\gamma}$ larger at last scattering surface.
% %\end{itemize}




%------------------------------------------------


%\begin{figure}[h]
 %   \centering
  %  \begin{subfigure}{0.34\textwidth}
   % \includegraphics[width=0.9\linewidth]{theo_plots/momentum_constraint_ratio_k0_0pt1.pdf}
    %\end{subfigure}
    %\begin{subfigure}{0.34\textwidth}
    %\includegraphics[width=0.9\linewidth]{theo_plots/momentum_constraint_ratio_k0_m0pt4.pdf}
    %\end{subfigure}
    %\begin{subfigure}{0.34\textwidth}
    %\includegraphics[width=0.9\linewidth]{theo_plots/momentum_constraint_ratio_k1_0pt1.pdf}
    %\end{subfigure}
    %\begin{subfigure}{0.34\textwidth}
    %\includegraphics[width=0.9\linewidth]{theo_plots/momentum_constraint_ratio_k1_m0pt4.pdf}
    %\end{subfigure}
    %\begin{subfigure}{0.34\textwidth}
    %\includegraphics[width=0.9\linewidth]{theo_plots/momentum_constraint_ratio_k2_0pt1.pdf}
    %\end{subfigure}
    %\begin{subfigure}{0.34\textwidth}
    %\includegraphics[width=0.9\linewidth]{theo_plots/momentum_constraint_ratio_k2_m0pt4.pdf}
    %\end{subfigure}
    %\begin{subfigure}{0.34\textwidth}
    %\includegraphics[width=0.9\linewidth]{theo_plots/momentum_constraint_ratio_k3_0pt1.pdf}
    %\end{subfigure}
    %\begin{subfigure}{0.34\textwidth}
    %\includegraphics[width=0.9\linewidth]{theo_plots/momentum_constraint_ratio_k3_m0pt4.pdf}
    %\end{subfigure}
    %\begin{subfigure}{0.34\textwidth}
    %\includegraphics[width=0.9\linewidth]{theo_plots/momentum_constraint_ratio_k4_0pt1.pdf}
    %\end{subfigure}
    %\begin{subfigure}{0.34\textwidth}
    %\includegraphics[width=0.9\linewidth]{theo_plots/momentum_constraint_ratio_k4_m0pt4.pdf}
    %\end{subfigure}
    %\caption{Upper panel of each pair: ratio of the purely non-GR term $\mathcal{G}\mathcal{H}\Psi$ to the sum of the matter and radiation source terms in the momentum constraint equation, shown in on the left for power law $n = 0.1$, and the on the right for $n = -0.4$. The perturbations are shown (in vertical descending order) for $\log{k/{\rm Mpc}^{-1}} = \left\lbrace -5, -4, -3, -2, -1\right\rbrace$. The momentum constraint equation governs the evolution of $\Psi$, and therefore of $\Phi$ once a slip relation is supplied. Lower panel of each pair: the effect of that $\mathcal{G}$ PPNC function on $\Phi + \Psi$, which is the total ``potential'' experienced by CMB photons, as a function of $a$. The presence of a large $\mathcal{G}$ drives this sum far away from the best-fit $\Lambda$CDM case, and therefore $\bar{\alpha} = \bar{\gamma}$ provides a much better fit to the potential than $\bar{\alpha} \neq \bar{\gamma}$.}
    %\label{fig_momentum_constraint_Phi+Psi}
%\end{figure}

